Dynamic Causal Bayesian Optimization

This paper studies the problem of performing a sequence of optimal interventions in a causal dynamical system where both the target variable of interest and the inputs evolve over time. This problem arises in a variety of domains e.g. system biology and operational research. Dynamic Causal Bayesian Optimization (DCBO) brings together ideas from sequential decision making, causal inference and Gaussian process (GP) emulation. DCBO is useful in scenarios where all causal effects in a graph are changing over time. At every time step DCBO identifies a local optimal intervention by integrating both observational and past interventional data collected from the system. We give theoretical results detailing how one can transfer interventional information across time steps and define a dynamic causal GP model which can be used to quantify uncertainty and find optimal interventions in practice. We demonstrate how DCBO identifies optimal interventions faster than competing approaches in multiple settings and applications.

==> figures/fig_sections/DAG_experiments.tex <==
\begin{figure*}[ht!]
\centering
\includegraphics[width=0.7\textwidth]{figures/graphs.eps}
\captionof{figure}{Another figure}
\label{fig:dag_experiments}
\end{figure*}

==> figures/fig_sections/fig_notation_plot.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/notation_plot.eps}
    \caption{Unrolling}
    \label{fig:notation_plot}
\end{figure*}



==> figures/fig_sections/main_nonstationary_synthetic_figure.tex <==
\begin{figure*}[ht!]
  \begin{minipage}{.3\textwidth}
        % Causal graphical model
        %\centering
        %\includegraphics[width =0.7\textwidth]{figures/synthetic/synthetic_example_cgm.eps}
        % Structural equation model
        %\begin{align*}
            % X_t &= f(X_{t-1}, \varepsilon_X) \\
            % Z_t &= g(Z_{t-1},X_t,\varepsilon_Z) \\
            % Y_t &= h(Y_{t-1},Z_t,\varepsilon_Y)
        %    X_t &= x_{t-1} +  \epsilon_X \\
        %    Z_t &= \exp(-X_{t}) + z_{t-1} + \epsilon_Z \\
        %    Y_t &= \cos(Z_{t}) - \exp \left (\frac{Z_t}{20} \right) + y_{t-1} + % \epsilon_Y
        %\end{align*}
    \includegraphics[width =0.9\textwidth]{figures/synthetic/nonstationary_synthetic_example_cgm.eps}
  \end{minipage}%
  \begin{minipage}{.7\textwidth}
        \centering
        \includegraphics[width =\textwidth]{figures/synthetic/joint_fig_synthetic.pdf}
        % \caption{Optimal sequence of interventions on our toy model.}
  \end{minipage}
  \caption{\nd{write}}
\end{figure*}

==> figures/fig_sections/main_synthetic_figure.tex <==
\begin{figure*}[ht!]
  \begin{minipage}{.3\textwidth}
        % Causal graphical model
        %\centering
        %\includegraphics[width =0.7\textwidth]{figures/synthetic/synthetic_example_cgm.eps}
        % Structural equation model
        %\begin{align*}
            % X_t &= f(X_{t-1}, \varepsilon_X) \\
            % Z_t &= g(Z_{t-1},X_t,\varepsilon_Z) \\
            % Y_t &= h(Y_{t-1},Z_t,\varepsilon_Y)
        %    X_t &= x_{t-1} +  \epsilon_X \\
        %    Z_t &= \exp(-X_{t}) + z_{t-1} + \epsilon_Z \\
        %    Y_t &= \cos(Z_{t}) - \exp \left (\frac{Z_t}{20} \right) + y_{t-1} + % \epsilon_Y
        %\end{align*}
    \includegraphics[width =0.9\textwidth]{figures/synthetic/toy_sem.png}
  \end{minipage}%
  \begin{minipage}{.7\textwidth}
        \centering
        \includegraphics[width =\textwidth]{figures/synthetic/joint_fig_synthetic.pdf}
        % \caption{Optimal sequence of interventions on our toy model.}
  \end{minipage}
  \caption{Toy example. \textit{Left}: \DAG and \sem. \textit{Right, upper row}: Objective functions for different intervention sets at different time steps. The red cross indicates the optimal intervention set and level. \textit{Right, middle row}: Posterior \gptext model obtained with \our and the benchmarks. \textit{Right, lower row}: Convergence of \our and benchmarks across different initializations of $\dataset^I$. The red line gives the optimal $\Yt$ at every time step.}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/alg.tex <==
\begin{figure}
\begin{minipage}{.55\textwidth}
 \scalebox{0.90}{
\begin{algorithm}[H]
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	\KwData{$\dataset^O$, $\{\DIntXstzero\}_{s \in \{0,\dots, |\missets_0|\}}$, $\graph_{0:T}$, 
	$P$. }
	\KwResult{Optimal intervention path $\{\Xst^\star, \xst^\star, y_t^\star\}_{t = 1}^T$}
	\textbf{Initialise}: $\missets$, $\dataset^I_0$ and initial optimal $\DIopt = \emptyset$.\\
	\For{$t = 0, \dots, T$}{ 
	1. Initialise dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\mathcal{D}^I_{\star,t-1}$ if $t>0$. \\
	2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$ \\
	\For{$p = 1, \dots, P$}{
	1. Compute $\EIst(\x)$ for each $\Xst \in \missets_t$.\\
	2. Obtain $(s^\star, \alpha^\star)$ \\
	3. Intervene and augment $\DIntXsstar$ \\
	4. Update posterior for $f_{s=s^\star, t}$
    }
    3. Return the optimal intervention $(\Xst^\star, \xst^\star)$\\
    4. Append optimal interventional data $\mathcal{D}^I_{\star,t} = \mathcal{D}^I_{\star,t-1} \cup ((\Xst^\star, \xst^\star), y^\star_t)$
	}
	\caption{\our}
	\label{alg:dcbo_alg}
\end{algorithm}
}
\end{minipage}

\begin{minipage}{.45\textwidth}



% \includegraphics[width=0.9\linewidth]{figures/graphs_vertical.eps}
% \caption{\DAG{s} used in the experimental sessions for the real and synthetic data.}
% \label{fig:dag_experiments}

\input{figures/experimental_dags}


\end{minipage}
\end{figure}

% \begin{algorithm}[t]
% 	\SetKwInOut{Input}{input}
% 	\SetKwInOut{Output}{output}
% 	\KwData{$\dataset^O$, $\{\DIntXstzero\}_{s \in \{0,\dots, |\missets_0|\}}$, $\graph_{0:T}$, 
% 	$P$. }
% 	\KwResult{Optimal intervention path $\{\Xst^\star, \xst^\star, y_t^\star\}_{t = 1}^T$}
% 	\textbf{Initialise}: $\missets$, $\dataset^I_0$ and initial optimal $\DIopt = \emptyset$.

% 	\For{t = 0, \dots, T}{\\ 
% 	1. Initialize dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\DIopt_{t-1}$ if $t>0$. \\
% 	2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$ \\
% 	\For{p = 1, \dots, P}{
% 	1. Compute $\EIst(\x)$ for each $\Xst \in \missets_t$.\\
% 	2. Obtain $(s^\star, \alpha^\star)$.\\
% 	3. Intervene and augment $\DIntXsstar$.\\
% 	4. Update posterior for $f_{s=s^\star, t}$
%     }
%     3. Return the optimal intervention $(\Xst^\star, \xst^\star)$.\\
%     4. Append optimal interventional data $\DIopt_t = \DIopt_{t-1} \cup ((\Xst^\star, \xst^\star), y^\star_t)$.
% 	}
% 	\caption{Dynamic Causal Bayesian Optimisation (\our)}
% 	\label{alg:dcbo_alg}
% \end{algorithm}

% 	Compute $\epsilon$ and sample $u \sim \mathcal{U}(0, 1)$.
% 	\If{$\epsilon > u$}{(Observe) \\
% 	1. Collect new observations $\mat{v}_t$. \\
% 	2. Augment $\dataset^O_t = \observations \cup \{\mat{v}_t\}$.\\
% 	3. Update prior surrogate models. 
% 	}
% 	\Else{(Intervene)\\
	%\; 1. Initialize dynamic causal \gptext models for all $\Xst \in \missets_t$ using $\DIopt_{t-1}$ if $t>0$.
	%2. Initialise interventional dataset $\{\DIntXst\}_{s \in \{0,\dots, |\missets_t|\}}$.

==> sections/connections_old.tex <==
\subsection{Connections}

The problem setup we study differs from those considered by both \cbo \cite{cbo} and \abo \cite{abo}. In this section we draw the links between these methods highlighting the reasons why \our is needed to solve the problem in \eq \eqref{eq:dcgo}. See \fig \ref{fig:map_methods} for a graphical representation of the relationship between \our and alternative optimization methods. A thorough discussion is included in the appendix (\S X).

\textbf{\cbo algorithm} \cbo tackles the causal dimension of the \dgo problem but not the temporal dimension. While it can be used to find optimal interventions to perform in a \DAG, this algorithm addresses static settings where variables in $\graph$ are i.i.d. across time steps, \ie $p(\mat{V}_t) = p(\mat{V})\text{,}\forall t$, and only one static target variable exists. For instance, \cbo can be used to find the optimal intervention for $Y$ in \fig \ref{fig:map_methods}, plate (b). Finding an optimal sequence of interventions for the \DAG in \fig \ref{fig:map_methods} plate (d) requires running \cbo for $T$ times optimizing $\Yt$ at each time step. In doing that \cbo re-initializes all surrogate models at every $t$ thus loosing all the information collected from previous interventions and not accounting for how the previously taken interventions have changed the system.

\textbf{\abo algorithm} \abo addresses dynamic settings but does not account for the causal relationships among variables. As done by \bo, \abo finds the optimal intervention values by breaking the causal dependencies among the inputs and intervening simultaneously on all of them thus setting $\Xst = \Xt$ for all $t$. Additionally, considering the inputs as fixed and not as random variables, \abo does not account for their temporal evolution (see \DAG (c) of \fig \ref{fig:map_methods}). Furthermore, \abo considers a continuous time space and places a surrogate model on $\Yt = f(\x, t)$. Considering a spatio-temporal \gptext allows \abo to predict the objective function ahead in time and track the evolution of the optimum. This is useful when the objective function rate of change over time is slow to gather enough samples to learn the relationships in space and time. In our discrete time setting this condition is equivalent to ask that the objective functions for different interventions do not change overtime. While this can be true in some stationary settings, it might not be the case in non stationary setting where both the \DAG and the \sem evolve overtime. In this settings \abo convergence is significantly slower.  

\our addresses both \cbo and \abo shortcomings. \our considers a different objective function at every time step, incorporates prior interventional information in the objective function and limits the search space at every time step based on the topology of the $\graph$. In addition, through the causal graph, \our imposes additional structure on the surrogate models. This allows \our to better track the dynamic of the objective function and deal with sharp changes in the objectives. \our is thus a framework that can be practically used for sequential decision making in a variety of applications.

\nd{Have to compare and contrast to reinforcement learning.}
